LGCC: Enhancing Flow Matching Based Text-Guided Image Editing with Local Gaussian Coupling and Context Consistency

Recent advancements have demonstrated the great potential of flow matching-based Multimodal Large Language Models (MLLMs) in image editing. However, state-of-the-art works like BAGEL face limitations, including detail degradation, content inconsistency, and inefficiency due to their reliance on random noise initialization. To address these issues, we propose LGCC, a novel framework with two key components: Local Gaussian Noise Coupling (LGNC) and Content Consistency Loss (CCL). LGNC preserves spatial details by modeling target image embeddings and their locally perturbed counterparts as coupled pairs, while CCL ensures semantic alignment between edit instructions and image modifications, preventing unintended content removal. By integrating LGCC with the BAGEL pre-trained model via curriculum learning, we significantly reduce inference steps, improving local detail scores on I2EBench by 1.60% and overall scores by 0.53%. LGCC achieves 3x -- 5x speedup for lightweight editing and 2x for universal editing, requiring only 40% -- 50% of the inference time of BAGEL or Flux. These results demonstrate LGCC's ability to preserve detail, maintain contextual integrity, and enhance inference speed, offering a cost-efficient solution without compromising editing quality.

==> others.tex <==

%  3.5 Inference and Image Generation

%  3.5.1 ODE-Free Sampling

% A major advantage of our explicit Gaussian coupling is the ability to perform inference without solving ODEs. During inference, given input image $\mathbf{I}_0$ and text $\mathbf{t}$, we:

% 1. Extract features: $\mathbf{z}_{\text{text}}, \mathbf{z}_{\text{vit}}, \mathbf{z}_{\text{src}}$
% 2. Sample noise: $\boldsymbol{\epsilon}_{\text{tgt}} \sim \mathcal{N}(0, \sigma^2 \mathbf{I})$
% 3. Create noisy target: $\mathbf{z}_{\text{tgt}}^{(0)} = \boldsymbol{\epsilon}_{\text{tgt}}$ (initialized as pure noise)
% 4. Form input: $\mathbf{z}_{\text{pack}} = [\mathbf{z}_{\text{text}}, \mathbf{z}_{\text{vit}}, \mathbf{z}_{\text{src}}, \mathbf{z}_{\text{tgt}}^{(0)}]$
% 5. Predict: $\mathbf{v}_0 = \text{Qwen2}(\mathbf{z}_{\text{pack}}, 0)$
% 6. Generate: $\mathbf{z}_{\text{tgt}} = \mathbf{z}_{\text{tgt}}^{(0)} + \mathbf{v}_0$
% 7. Decode: $\mathbf{I}_1 = \text{FluxDecoder}(\mathbf{z}_{\text{tgt}})$

% This single forward pass achieves high-quality editing results, dramatically reducing inference time compared to iterative sampling methods.

%  3.5.2 Multi-Step Refinement (Optional)

% For applications requiring higher precision, we optionally employ a multi-step procedure with explicit integration:

% $\mathbf{z}_{\text{tgt}}^{(k+1)} = \mathbf{z}_{\text{tgt}}^{(k)} + \Delta t \cdot \mathbf{v}_{t_k}$

% where $\mathbf{v}_{t_k} = \text{Qwen2}([\mathbf{z}_{\text{text}}, \mathbf{z}_{\text{vit}}, \mathbf{z}_{\text{src}}, \mathbf{z}_{\text{tgt}}^{(k)}], t_k)$.

% Due to the straight trajectory property, even 2-5 steps achieve results comparable to methods requiring 50+ steps.

%  3.6 Training Strategy

%  3.6.1 Data Preparation

% We train on paired datasets where each sample consists of:
% - Original image $\mathbf{I}_0$
% - Editing instruction text $\mathbf{t}$
% - Target edited image $\mathbf{I}_1$

% During training, Gaussian noise is added on-the-fly to both VAE features:
% - $\mathbf{z}_{\text{src}}^{(0)} = \mathbf{z}_{\text{src}} + \boldsymbol{\epsilon}_{\text{src}}$
% - $\mathbf{z}_{\text{tgt}}^{(0)} = \mathbf{z}_{\text{tgt}} + \boldsymbol{\epsilon}_{\text{tgt}}$

%  3.6.2 Explicit Loss Computation

% The training objective leverages the explicit form of our coupling:

% $\mathcal{L}_{total} = \mathbb{E}_{t \sim U(0,1)} \left[ \left\| \text{Qwen2}(\mathbf{z}_{\text{pack}}, t)_{\text{target}} - (-\boldsymbol{\epsilon}_{\text{tgt}}) \right\|^2 \right]$

% where $\mathbf{z}_{\text{pack}} = [\mathbf{z}_{\text{text}}, \mathbf{z}_{\text{vit}}, \mathbf{z}_{\text{src}}^{(0)}, \mathbf{z}_{\text{tgt}}^{(0)}]$ and the subscript "target" denotes extraction of the target VAE feature portion from the Qwen2 output.



% \subsection{Problem Setup}


% Let $x_1 \in \mathbb{R}^d$ denote a **target image** in the data distribution $\mu$, and $x_0 \in \mathbb{R}^d$ be its corresponding source point in a structured noise distribution $\nu$. In typical OFM settings, one seeks an optimal coupling $\pi(x_0, x_1)$ between these distributions via an explicit or implicit transport plan. Instead, we **parameterize the coupling** directly using a **deterministic embedding function** $f_\phi: \mathbb{R}^d \rightarrow \mathbb{R}^d$ (e.g., a CLIP or VAE encoder), such that:

% $$
% x_0 = f_\phi(x_1) + \epsilon, \quad \epsilon \sim \mathcal{N}(0, \sigma^2 I)
% $$

% This formulation assumes that the optimal source point for editing $x_1$ lies near its embedding plus small Gaussian perturbation. This eliminates the need for Sinkhorn-based coupling and ensures consistent semantic alignment between noisy and clean image domains.

%  3.2 Optimal Flow via Convex Potential

% Following OFM theory, we model the transport from $x_0 \sim \nu$ to $x_1 \sim \mu$ via a **vector field** that is the **gradient of a convex potential function** $\phi_\theta: \mathbb{R}^d \rightarrow \mathbb{R}$. We parameterize $\phi_\theta$ using an **Input Convex Neural Network (ICNN)** to ensure the convexity constraint is satisfied. The transport map is then:

% $$
% T(x_0) = x_0 + \nabla \phi_\theta(x_0)
% $$

% During training, we minimize the flow matching objective:

% $$
% \mathcal{L}_{\text{OFM}} = \mathbb{E}_{x_1 \sim \mu, \epsilon \sim \mathcal{N}(0, \sigma^2 I)} \left[ \left\| \nabla \phi_\theta(f_\phi(x_1) + \epsilon) - (x_1 - f_\phi(x_1) - \epsilon) \right\|^2 \right]
% $$

% This loss encourages the gradient of the learned potential to match the true optimal direction from noise to image.

%  3.3 One-Step Image Editing Inference

% Given an input image $x_{\text{input}}$ and an editing instruction $t$ (e.g., a caption or prompt), we first encode the image using a conditional embedding model:

% $$
% z_1 = f_\phi(x_{\text{input}}, t)
% $$

% To sample a source point in noise space, we add Gaussian noise:

% $$
% x_0 = z_1 + \epsilon, \quad \epsilon \sim \mathcal{N}(0, \sigma^2 I)
% $$

% We then apply a **single-step transport** via the learned ICNN:

% $$
% x_{\text{edited}} = x_0 + \nabla \phi_\theta(x_0)
% $$

% Optionally, a lightweight decoder (e.g., a shallow U-Net or VAE decoder) is used to transform $x_{\text{edited}}$ back into pixel space. This inference process is **extremely fast**, requires **no iterative sampling**, and produces high-quality, semantically aligned outputs in a **single forward pass**.

%  3.4 Conditional Image Editing via Embedding Guidance

% To incorporate editing instructions, we condition both $f_\phi$ and $\phi_\theta$ on text prompts. This enables **instructional control** over the transport map, allowing for edits such as style transfer, object replacement, or color adjustment.

% In practice, we use a joint vision-language embedding (e.g., CLIP or SigLIP) to encode both $x_1$ and the instruction $t$, ensuring **semantic grounding** and **edit relevance**.


